SmartPM: Automatic Adaptation of Dynamic Processes at Run-Time

The research activity outlined in this PhD thesis is devoted to define a general approach, a concrete architecture and a prototype Process Management System (PMS) for the automated adaptation of dynamic processes at run-time, on the basis of a declarative specification of process tasks and relying on well-established reasoning about actions and planning techniques. The purpose is to demonstrate that the combination of procedural and imperative models with declarative elements, along with the exploitation of techniques from the field of artificial intelligence (AI), such as Situation Calculus, IndiGolog and automated planning, can increase the ability of existing PMSs of supporting dynamic processes. To this end, a prototype PMS named SmartPM, which is specifically tailored for supporting collaborative work of process participants during pervasive scenarios, has been developed. The adaptation mechanism deployed on SmartPM is based on execution monitoring for detecting failures at run-time, which does not require the definition of the adaptation strategy in the process itself (as most of the current approaches do), and on automatic planning techniques for the synthesis of the recovery procedure.

==> 1-Introduction/challenges.tex <==
\section{Challenges and Requirements for the \smartpm Development}
\label{sec:introduction-challenges}

The \smartpm prototype system was born in the range of the WORKPAD European research project~\cite{IEEE2008}, which concerned to devise an high-level architecture for emergency management systems. The WORKPAD architecture is specifically tailored for supporting collaborative work of human operators during disaster scenarios, where different teams, belonging to different
organizations, need to collaborate in order to reach a common goal.

With the WORKPAD project we studied the potential benefits coming from the application of process management principles and practices to emergency management settings. Providing coordination support by means of an adequate process management approach allows promoting a collaboration-aware and process-aware methodology, still preserving the autonomy of individual mobile operators. Business processes are well suited for coordinating services and operators to achieve a certain goal, as they enable to define structured and guided interactions between users and the environment.

However, although the exploitation of PMSs to support the enactment of processes in pervasive and mobile scenarios represents a promising and helpful approach, on the other hand moving to a pervasive dynamic environment introduces additional challenges and requirements, due to wireless networking, device mobility and high variability of the working environment.

In particular, emergency operators act in a complex pervasive environment, highly dynamic in space and time. The \emph{operational context} is given by the physical environment (i.e., the affected area) and by other heterogeneous contextual information, including absolute and relative positioning of mobile resources, process execution status, resource availability, etc. As changes in the operational context may occur unpredictably and at any time (a landslide or a collapse may modify the operational theater, a software or hardware resource may disconnect or fail, etc.), a software system designed to support coordination should be able to react to those changes and properly adapt and modify its behavior.

To deal with those challenges is exactly the main purpose of the \smartpm prototype system.





%PERCHE' HO USATO INDIGOLOG E NON PETRI NET O ALTRI FORMALISMI?

%Note that, as shown in Fig.~\ref{fig:fig_anatomy}(a), our approach treats each task as a ``black box'' and no assumption is made about its internal behavior (we consider the task execution as an instantaneous activity).\vspace{-0.5em}


\begin{comment}
The \mobidis system is under development in the context of the
European-funded project called WORKPAD, which concerns devising a
two-level software infrastructure for supporting rescue operators of
different organisations during operations of emergency
management~\cite{IC2008}. In the context of this project, the whole
\mobidis system has been devised in cooperation with real end users,
specifically ``Protezione Civile della Calabria'' (Civil Protection
and Homeland Security of Calabria). Indeed, the rest of this thesis
will explain the various introduced techniques through examples
stemming from emergency management. But its exploitation comprises
many other possible pervasive scenarios (such as those described
above). According to the Human-Computer Interaction methodology
different prototypes have been proposed to users who fed back with
comments~\cite{H_C_dL_M_M_B_S@KTP09,H_C_dL_M_M_B_S@HCI09}. At each
iteration cycle the prototype has been refined according to such
feedbacks till meeting finally the complete users' satisfaction.

From the analysis with final users, we learnt that processes for
pervasive scenarios are highly critical and time demanding as well
as they often need to be carried out within strictly specified
deadlines. Therefore, it is unapplicable to use a pull mechanism for
task assignment where \mobidis would assign every task to all
process participants qualified for it, letting them decide
autonomously what task to execute as next. Consequently, \mobidis
aims at improving the overall effectiveness of the process execution
by assigning tasks to just one member and, vice versa, by assigning
at most one task to members.

Moreover, these processes are created in an ad-hoc manner upon the
occurrence of certain events. These processes are designed starting
from provided templates or simple textual guidelines on demand. In
the light of that, these processes are used only once for the
specific setting for which they were created; later, they will not
be used anymore. Moreover, process participants are asked to face
one situation and, hence, they take part in only one process
simultaneously.
\end{comment} 

==> 2-State_of_the_Art/WfNet.tex <==
\subsection{Workflow Nets}
\label{subsec:state_of_the_art-soa_modeling_languages-WFnet}

One of the most famous modeling languages used for defining process specifications is the language provided by the \emph{Workflow nets}~\cite{vanderAllst@WorkflowNets1998}, a subclass of the well-known \emph{Petri
Nets}~\cite{petriNet}. A Petri net is a directed bipartite graph~\cite{diestel2005graph} whose vertices can be divided into two disjoint finite sets consisting of \emph{places} and \emph{transitions}. Every arc of a Petri net connects a place to a transition or viceversa. Formally, a Petri net is a three tuple, where:
\begin{itemize}[itemsep=1pt,parsep=1pt,topsep=0.5pt]
\item \emph{S} is a finite set of places;
\item \emph{T} is a finite set of transitions;
\item  $W : (S x T) \cup (T x S) \rightarrow \mathbb{N}$ is a multiset of arcs, i.e., it assigns to each arc a non-negative integer arc multiplicity. Note that no arc may connect two places or two transitions.
\end{itemize}

From a graphical point of view, places are represented by circles and transitions by rectangles. Places in a Petri net may contain a discrete number of marks called \emph{tokens}. Any distribution of tokens over the places will represent a configuration of the net called a \emph{marking}. Formally, a marking of a Petri net is a multiset of its places, i.e., a mapping $M : S \rightarrow \mathbb{N}$. We say the marking assigns to each place a number of tokens. A transition of a Petri net may \emph{fire} whenever there are sufficient tokens at the start of all input arcs; when it fires, it consumes these tokens, and places tokens at the end of all output arcs. A firing is atomic, i.e., a single non-interruptible step.

\begin{figure}
\begin{center}
 \includegraphics[width = 0.8\textwidth]{2-State_of_the_Art/images/petri_net_ex.pdf}
\end{center}
\caption{An example of Petri Net} \label{fig:fig_state_of_the_art_petrinet}
\end{figure}

Figure~\ref{fig:fig_state_of_the_art_petrinet} shows an example of a Petri net; the black dots on the places represent tokens and their location. An \emph{input place} of a transition $t$ is such that it has an outgoing arc toward $t$, and vice versa an \emph{output place} of $t$ has ingoing arcs from $t$. A certain transition $t$ is said to fire if for each input place one token is removed and one token is placed in each output place. Of course, a transition can fire only if it is \emph{enabled}, that is each input place contains at least one token.



In the context of process management, transitions represent
activities and their firing represent their execution. Places and
connecting arcs represent the process instance state as well as the
process constraints. For instance, in the Petri Net above, the two
tokens' location identify that transitions \emph{Send
Acknowledgement} and \emph{Request and check payment} are enabled.
Therefore, the corresponding activities are ready to be assigned to
participants and executed.



Workflow nets allow one to define unambiguous specifications,
formally reason on them as well as to check for specific properties.

For the sake of brevity, here we introduce formally only an
extension by Kurt Jensen~\cite{JensenBook}, named \emph{coloured
Petri net}, which is better tailored to process management. Coloured
Petri Nets introduces the association of ``colours'' to tokens. Data
types associated to tokens are called colour sets, where a colour
set of a token represents the set of values that tokens may have.
Like in programming languages data values of a certain type are
associate to variables, in coloured petri nets colours of a certain
colour set are associated to tokens. Colours are meant to hold
application data, including process instance identifiers. Places may
have a different colour set, since some additional data can become
available while tokens are passing through the net (i.e., activities
are executed).

A \textbf{coloured Petri net} is a tuple $(\Sigma,P,T,A,N,C,G,E,I)$
where:
\begin{itemize}
  \item $\Sigma$ is a finite set of non-empty types, called colour
  sets
  \item $P$ is a finite set of places
  \item $T$ is a finite set of transitions
  \item $A$ is a finite set of arc identifiers, such that $P \cap T
  = P \cap A = T \cap A = \emptyset$
  \item $N : A \rightarrow (P \times T) \cup (T \times P)$ is a node
  function mapping each arc identifier to a pair $(start_node,
  end_node)$ of the arc.
  \item $C: P \rightarrow \Sigma$ is a colour function that
  associates each place with a colour set.
  \item $G: T \rightarrow BoolExpr$ is a guard function that maps
  each transition to a boolean expression $BoolExpr$ over the token
  colour.
  \item $E: A \rightarrow Expr$ is an arc expression that evaluates
  to a multi-set over the colour set of the place
  \item $I$ is an initial \emph{marking} of the colour Petri Net,
  the initial position of possible tokens with their respective
  values.
\end{itemize}

In coloured Petri nets, the enabling of a certain transition is
determined not only by the existence of tokens on the input places
but also by the values of the colour sets of such tokens. A
transition is enabled if the guard function for that transition is
evaluated as true and the arch expression is satisfied. When a
transition fires, the respective tokens are removed from the input
places and others are placed in the output places guided by,
respectively, the arc expression of the ingoing and outgoing edge.

In order to represent the dynamic status of Colour Petri Nets, there
exists a function \emph{marking} which returns, for each place $p
\in P$ and for each possible colour value $v \in C(p)$, the number
of tokens in $p$ with value $v$:

Let be $PN = (\Sigma,P,T,A,N,C,G,E,I)$. For all $p_i \in P$, let
$\sigma_{p_i}$ be s.t. $C(p_i) = \sigma_i$. For all $p_i$ there
exists a function $M_{p_i}: \sigma_{p_i} \rightarrow \mathbb{N}$. A
\textbf{marking function} for $PN$ is defined as follows:
\begin{displaymath}
M(p,q) = \left\{ \begin{array}{ll}
M_p(q) & if~\sigma_{p_i} = C(p_i)~\vee~q \in \sigma_{p_i}\\
0 & otherwise
\end{array} \right.
\end{displaymath}

Petri nets should have specific structural restrictions in order to
be properly used for process management. In that case, they are
named workflow nets:

A Petri Net $PN = \Sigma,P,T,A,N,C,G,E,I)$ is called
\textbf{workflow net} iff the following conditions hold:
\begin{itemize}
  \item There is a distinguished place place $i \in P$, named
  initial place, that has no incoming edge.
  \item There is a distinguished place place $o \in P$, named
  final place, that has no outgoing edge.
  \item Every place and transition is located on a firing path from
  the initial to the final place.
\end{itemize}

Papers~\cite{vdA@Circuits98,vdA@BPM2000} has studied the problem of
checking the soundness. Indeed, a process definition is said to be
sound if any run-time execution of its cases may not lead to
situations of deadlock (the process is not completed but no activity
can be executed) or livelocks (the process cycles executing
infinitely always the same activities and never terminates). In
those papers soundness is defined as follows:\footnote{The state of
a workflow net is here defined in term of the associated marking
function. If $\exists q \in C(o),M(o,q) \geq 0$, then  $M \geq o$.
In addition, if $M \geq 0$ and $\forall p \in P\setminus\{o\}$
holds, then $M = {o}$}
\begin{definition}[Soundness]
\label{def:soundness}
 Let \mbox{$PN = (\Sigma,P,T,A,N,C,G,E,I)$} be a Workflow Net
with initial place $i$ and final place $o$. $PN$ is structurally
sound if and only if the following properties hold:
\begin{description}
  \item[Termination.] For every state $M$
  reachable from $i$ there exists a firing
  sequence leading from $M$ to $o$:
  \begin{displaymath}
    \forall M, i \arrowstar M \Rightarrow M \arrowstar o
  \end{displaymath}
  \item[Proper termination.] State $o$ is the only state reachable from state $i$ with at least one token
  in place $o$:
  \begin{displaymath}
    \forall M, i \arrowstar M \cup M \geq o \Rightarrow M = o
  \end{displaymath}
  \item[No dead transitions.] Each transition $t \in  T$ can contribute
  to at least one process instance:
  \begin{displaymath}
    \forall t \in T, \exists M, M', i \arrowstar M \arrow{t} M'
  \end{displaymath}
\end{description}
\end{definition}

In some cases designers are only interested in checking whether a
process specification allows to reach each defined activity for some
execution. When the final state is reached, there can be tokens left
in the net, maybe stuck in deadlock situations. For these concerns,
the soundness criterion appears to be too restrictive. In the light
of this, paper~\cite{d_R@CAISE2001} has introduced the notion of
Relaxed Soundness:
\begin{definition}[Relaxed Soundness]
\label{def:relaxedsoundness}
 Let \mbox{$PN = (\Sigma,P,T,A,N,C,G,E,I)$} be a Workflow Net
with initial place $i$ and final place $o$. $PN$ is relaxed sound if
and only if each transition participates in at least one legal
process instance starting from the initial state and reaching the
final one:
\begin{displaymath}
    \forall t \in T, \exists M, M' : i \arrowstar M \arrow{t} M'
    \arrowstar o
\end{displaymath}
\end{definition}


==> 2-State_of_the_Art/soa_modeling_languages.tex <==
\section{Process Modeling Languages}
\label{soa_modeling_languages}

To discuss alternative process designs with stakeholders and to evaluate the designed processes in respect to these goals, process knowledge must be first captured in business \emph{process models}. The purpose of process modeling is to ``produce an abstraction of a process (model) that serves as a basis for the process specification''. Process models can be used for improved human understanding of operations within a domain, or to assist with analysis or re-engineering~\cite{cichocki1997workflow}.

Process modeling is the first and most important step in BPM lifecycle~\cite{vanderAalst@BPM2003}, which intends to separate process logic from application logic, such that the underlying business process can be automated. Typically, process logic is implemented and managed through a PMS and application logic through underlying application components~\cite{Sadiq@BIS2007}.



%A wide range of process modelling approaches has been proposed over time, ranging from simple flowcharts to advanced variants of Petri nets with high expressive power.

In the research literature, there have been some investigations that analyzed process modeling languages on the basis of different comparison techniques. For example, in~\cite{Kaschek@BIS2006} is presented a framework for selecting appropriate process modeling tools based on some heuristics collected from business domain experts. Such heuristics are used to provide quantifiable measure for indicating preferences on modeling tools selection.

Finally, the work~\cite{Sedera@ECIS2003} presents an empirical study on process modeling success in industry, where success factors of process modeling are generalized from multiple case studies of industry applications and the measure for effective process modeling is derived. In particular,~\cite{Sedera@ECIS2003} analyzes the semantic richness of an appropriate ontology as the benchmark for comparing process modeling languages.

The focus of this Section is to analyze the existing modeling approaches and to investigate their degree of adaptation.

Since in the literature there are two most predominant formalisms on which process modeling languages are developed, namely \emph{graph-based formalism} (it has its root in graph theory) and \emph{rule-based formalism} (based mainly on formal logic), we decide to analyze these two kinds of modeling approach separately and then to provide a discussion.

%In the research literature, it has been found that there are two most predominant formalisms on which process modeling languages are developed, namely \emph{graph-based formalism} and \emph{rule-based formalism}~\cite{SadiqSurvey07}. In a graph-based modeling language, process definition is specified in graphical process models, where activities are represented as nodes, and control flow and data dependencies between activities as arcs. On the contrary, in a typical rule-based approach, process logic is abstracted into a set of rules, each of which is associated with one or more business activity, specifying properties of the activity such as the pre- and post-conditions of execution. At runtime, a rule inference engine examines data and control conditions and determines the best order for executing relevant business activities according to pre-defined rules.



%Sadiq:2007
%-------------------
% The origins of process modeling languages are quite diverse, although two dominant approaches can be observed; one based on graphical models, and the other based on rule specifications. However, at this time, there is no report in literature that specifically targets a comparative analysis of these two approaches, on aspects such as the relative areas of application, power of expression, and limitations.  We will present both a survey of the two approaches as well as a critical and comparative analysis.
%------------------
%Business process modeling is a complicated process and it is obvious that different modeling approaches have their strengths and weaknesses in different aspects due to the variety of their underlying formalisms. Some languages offer richer syntax sufficient to express most relevant business activities and their relationships in the process model, while some provide more generic modeling constructs which facilitate efficient verification of the process model at design time.

%Myers@1998
%-------------------
%The purpose of process modeling is to "produce an abstraction of a process (model) that serves as a basis for the workflow specification" [15]. Process models can be used for improved human understanding of operations within a domain, or to assist with analysis or re-engineering. Additionally, they can serve as the basis for automated workflow control. Process modeling as a discipline has been around for some time. To date, two main approaches have been defined [15]:
%.. Artifact-based modeling focuses on the objects (e.g., data or information) that are created, modified, and used within a process, along with their paths through a series of activities.
%.. Activity-based modeling focuses on the activities that are to be performed within a process, along with dependencies and constraints among them.
%The WfMC focuses on the activity-based paradigm for process modeling.

%Bucchiarone@SOCA2011
%--------------------
%The vast majority of these approaches can be characterized as rule-based, since they predefine rules on how to transform a basic process in extraordinary situations. Some approaches introduce transformation rules explicitly [5], [15], [19], others define process variants [10], [12], [11] or use aspect-oriented methodologies [14], [1], [11]. Rules are more general than built-in adaptation since, while being written at design time, they are applied to a targeted process at run time, when more information on the extraordinary situation and execution context is available. This also results in much better scalability. Rule-based approaches, however, still share a major drawback with built-in approaches. Since the ules are specified at design time, the designer has to choose a particular adaptation tactic for a certain extraordinary situation. At run time, it may happen that the tactic chosen is not applicable (e.g., if it requires the usage of a service that became unavailable), or a better tactic could be available (e.g., newly appeared services may allow for better recovery approaches). Maintaining an updated and consistent set of adaptation rules is a very time-consuming and error-prone task that requires profound knowledge of the execution environment, as well as advanced supporting tools. Moreover, sophisticated adaptation tactics usually require considerable amount of rules to be specified.
%----------------------
%Unlike rule-based approaches, our goal-based approach guarantees that if solutions exist they will be found automatically, without involving design activities by process analysts. In this regard, it overcomes the limitations of the rule-based approaches discussed above. Compared to other existing solutions, we also expect it to provide better flexibility, scalability and designer's productivity when applied to the business processes acting in extremely dynamic environments.

\input{2-State_of_the_Art/WfNet}

\input{2-State_of_the_Art/BPMN}



\subsection{Discussion}
\label{subsec:soa_Discussion_1} 
